SAID: A Control Protocol for Scalable and Adaptive Information Dissemination in ICN

Information dissemination applications (video, news, social media, etc.) with large number of receivers need to be efficient but also have limited loss tolerance. The new Information-Centric Networks (ICN) paradigm offers an alternative approach for reliably delivering data by naming content and exploiting data available at any intermediate point (e.g., caches). However, receivers are often heterogeneous, with widely varying receive rates. When using existing ICN congestion control mechanisms with in-sequence delivery, a particularly thorny problem of receivers going out-of-sync results in inefficiency and unfairness with heterogeneous receivers. We argue that separating reliability from congestion control leads to more scalable, efficient and fair data dissemination, and propose SAID, a Control Protocol for Scalable and Adaptive Information Dissemination in ICN. To maximize the amount of data transmitted at the first attempt, receivers request any next packet (ANP) of a flow instead of next-in-sequence packet, independent of the provider's transmit rate. This allows providers to transmit at an application-efficient rate, without being limited by the slower receivers. SAID ensures reliable delivery to all receivers eventually, by cooperative repair, while preserving privacy without unduly trusting other receivers.

==> ackerselection.tex <==
\vspace{-2mm}
\section{Provider Transmission Rate Control}
\label{sec-appendix-ackerselection}
The data-provider's sending rate is typically determined by application requirements.
%Different applications have different requirements on the sending rate at the data-provider.
Applications like audio/video streaming need a certain minimum rate for proper audio/video progression and might also have a limit on the maximum rate. However, certain other applications such as file delivery are more elastic and therefore the sender can find a balance between the average completion time and the network load (as illustrated be Fig.~\ref{fig:repair_throughput}).
\hide{
% Mayu: can add if space is available
Even if the application chooses a sending rate that is higher than all the receivers' bandwidth, it will not result in a congestion collapse. This is due to the fact that the packet will be ``dropped'' at the $1^{st}$ hop router of the data provider since the pending requests are consumed faster than their accumulation at that router.
}

%From Fig.~\ref{fig:repair_throughput}, we can see that if the sending rate is too low, the flow under-utilizes the network. Although the network load is low, the average completion time can be quite high. But when the sending rate becomes too high, a large portion of the data will have to be retransmitted by repair. The retransmission load becomes high and the average completion time might further increase if the repair causes congestion in the network.
%Since there are differences in the desired level of control over the sending rate from different applications, we believe it is appropriate to design it at the application layer (or at least allow applications to specify their desired level of control).
%For applications with a specific required rate, the data provider only needs to send the packets at that constant rate.
%The absence of pending requests at the $1^{st}$ hop router will result in transmission not making progress.
%Therefore, no matter how fast the data provider can send the data, the data will not cause congestion collapse in the network.

For general-purpose data transmission, we suggest the data provider send at the rate that the \emph{majority} of the receivers can receive. Therefore, those consumers can receive all of the data transmitted without much repair, % (or only repair a small part)
while the slower receivers (the \emph{minority}) will depend on the other receivers % (especially the majority)
for the missing packets.
However, the estimation of the receive rate of the majority is not easy either, because of the highly dynamic nature of network.
Therefore, instead of \emph{estimating} the receive rate for the majority directly,
we divide the task into two parts: 1) find a proper receiver (normally the slowest in the majority) as an \emph{ACKer} and 2) \emph{align} the content provider's sending rate to the ACKer's available bandwidth.
%This solution is similar to pgmcc\cite{pgmcc}.
Unlike pgmcc\cite{pgmcc}, the ACKer we pick is the slowest in the majority, not the slowest among \emph {all} the receivers.
This allows our solution be more efficient than pgmcc because we exploit the efficient repair capability in ICN.
Note that our solution can also align to the slowest receiver if the application demands it, but by having the ability to also align to a constant rate or to that of the majority, our solution is more flexible and can support different types of applications needs. % (see \S~\ref{sec-discussion}).

%\subsection{ACKer Selection}

A critical component of the mechanism is the selection of the
ACKer.
Due to the dynamic nature of the network, the slowest receiver in the majority might change from time to time.
Therefore, the provider should have the ability to change the ACKer based on network conditions.
But compared to the per-RTT estimation of sending rate, the ACKer selection can be made over a relatively longer time scale. The provider initiates the ACKer selection periodically.

\hide{
\subsubsection{Initiation phase}
Unlike some of the IP multicast protocols, \name does not adopt a session-initiation phase.
The provider starts to collect data concurrently with data dissemination.
%Thus, the provider has no information of the current receivers for the first period.
Therefore, when sending the first packet, the provider indicates that each consumer should respond with his unique ID in the flow to the provider.
For the second packet, the provider uses the receiver that responds first as the ACKer, since in the worst case scenario, there may be only one receiver.
Later, as the provider receives more ACKs for the first packet, he can elect the ACKer based on the latency until the end of the initiation period.
}

%\subsubsection{Periodic feedback}
Unlike some of the IP multicast protocols, \name does not adopt a session-initiation phase.
Instead, it relies on feedback sent by the receivers to the first packet in order to elect the initial ACKer.
%On receiving data for a period of time, the receivers are able to collect throughput statistics.
Periodically, the data provider triggers the collection of receiver statistics, by
% To reliably deliver the trigger information, we
piggy-backing a trigger packet containing the statistics collection range (start segment ID and end segment ID) for a period of time (\eg, a window).

%Multiple values need to be used to get the estimate of the available bandwidth at the receiver.
%The first is the number of packets received. This is a direct value to estimate the current receive rate.
The number of packets received can be used to estimate the current receive rate.
But receivers with an available bandwidth higher than the ACKer will all have the same receive count.
Therefore, we depend on  a second value: the number of received packets that were marked.
Faster receivers will receive fewer marked packets compared to the ACKer.
Different receivers might have received a slightly different number of packets, due to queueing at routers.
To better reflect the receive rate, we also take the last received packet into consideration.
%On receiving a statistics collection packet with a 'start' and 'end' range, every receiver encapsulates the number of packets received, the number of packets marked and the segment ID of last received packet into an Interest packet. The Interest packet has the flow ID as the prefix and the network knows how to reach the data provider since the provider already advertized the FIB of the flow ID.
On receiving the statistics from the receivers, the provider calculates the score of every receiver as
\begin{equation}\label{equ-acker-selection}
  S=\frac{ReceivePktCount - 0.5 \times MarkPktCount}{LastReceiveID - RangeStart}.
\end{equation}
We value a marked packet a being half as good as a normal packet, so as to space out the faster receivers. The receiver at rank $R$ will be elected as the new ACKer.
However, we believe that changing the ACKer frequently might affect the stability of the flow
%(the RTT of the ACKer might change).
and therefore only elect a new ACKer if the current ACKer is not in the range $R \pm R_{th}$.
But when the condition in the network or the receivers changes dramatically, a shift on the ACKer is inevitable.
%\jnote{Is ACKer shift removed? Is that OK?}
%Then, the publisher would have to select either a different ACKer.

Selecting a slower ACKer than the current one is relatively easy. Using Eq.~(\ref{equ-acker-selection}), we can select a slower receiver that has a lower receive count and higher mark count in proportion to their available bandwidth.
But selecting a faster ACKer is not straightforward since the new ACKer should be among the faster receivers who all receive at the same rate as the current ACKer.
The mark count in Eq.~(\ref{equ-acker-selection}) will take effect in this case.
Although the faster receivers have the same receive count as the ACKer, they have a lower mark count.

In the overall evaluation, each data provider picks the ACKer at $60\%\pm 5\%$, and resulted in around $60\%$ delivered on the first-attempt.














\hide{
\subsubsection{Selecting a slower ACKer}
Often a competing flow appears on a link closer to the root of the dissemination tree and thus many receivers' rate is lowered. If the ACKer is among the affected receivers, the window-based solution would adjust the throughput automatically. But if the ACKer is not affected, the flow needs to find a slower ACKer in order to have the sending rate match the new majority and to avoid wastage of resources and time on the repair phase. The departure of fast receivers can also cause a provider to try to select a slower ACKer.

Selecting a slower ACKer is relatively easy. The slower receivers always have a lower receive count and higher mark count in proportion to their available bandwidth. Using equation~\ref{equ-acker-selection}, we easily find a proper new ACKer.


\subsubsection{Select a faster ACKer}

The provider might also have to elect a faster ACKer due to the departure of slower subscribers or on completion of a competing flow. But selecting a faster ACKer is not straightforward since the new ACKer should be among the faster receivers who all receive at the same rate as the current ACKer.
The mark count in equation~\ref{equ-acker-selection} will take effect in this case.
Although the faster receivers have the same receive count as the ACKer, they have a lower mark count. If two receivers have the same score, we will order the receivers based on their response time. The receiver with lower RTT (who responds faster) is ranked higher since he will have higher throughput.

This estimation might not be accurate. But if we analyse the election in the long run, the selection of an ACKer that is not fast enough (but one that is faster than the current ACKer), will result in the provider trying to find an even faster ACKer subsequently in the next period.
If the new ACKer is too fast, the provider can easily find a slower one based on the slower ACKer selection means described above. The provider can gradually find a proper sending rate using this mechanism.


\subsection{ACKer Logic}
\label{sec-pubcontrol-acker}
%\mnote{we could move this to come after ACKer Selection and probably as the first part of the ACKer shift section}
%Jia: The "ask for all" logic will be used by the ACKer selection... Was struggling about this also.
Since every packet sent from the data provider will be received by multiple receivers, the data provider places the ACKer ID in every data packet to assign a proper ACKer for that packet. On receiving a packet with his own ID, that receiver sends an ACK back to the data provider. Using a congestion control model like TCP, a closed feedback loop is thus formed between sender
and the ACKer to align the sending rate to the ACKer's receive rate.

Unlike the communication model of the followers, the rate is controlled on the sender (content provider) side for the ACKer (and thereby the
'faster' receivers forming the majority). The ACKer is likely to receive \emph{all} the packets for that flow. This is also achieved by modifying an Interest packet. We still put the flow ID in the Content Name field but
utilize a flag bit to indicate to intermediate router to forward all the packets in the flow to that outgoing face.


\subsection{ACKer Switching Policy}
\begin{figure}[t!]
  \centering
  \includegraphics[width=0.4\textwidth]{figures/ACKerShift}\\
  \caption{Procedure of ACKer shift}\label{fig:ackershift}
\end{figure}



%See if we have better reason why we use an in-band ACKer notification but not like the info collection
% Mayutan: we need to avoid using he, if we use it, it might be better to use (s)he of just she, her and etc..
To ensure the reliable method to switch between the new and the old ACKer, we designed an in-band notification procedure.
The procedure is shown in Fig.~\ref{fig:ackershift}. When the data provider decides to shift to a new ACKer at time $t1$, he starts to send packets indicating that both the original ACKer and the new ACKer should provide feedback (ACK). Since the new ACKer is still using the follower logic, he may miss some of these packets especially if he has a lower available bandwidth (the dashed lines on the right). But the new ACKer will eventually receive a data packet with his ID in the ACKer list. This is the first time the new ACKer sees his ID in the ACKer list. He will first change the request type to ``all'' by sending a special Interest packet described in \S\ref{sec-pubcontrol-acker}, and then send an ACK to the packet from the data provider.
Both the request to ``all'' and the ACK will follow the same path towards the data provider. So at time $t2$, when the data provider receives the ACK from the new ACKer (segment number might be larger than $S1$), the provider can be sure that the new ACKer is using the ACKer logic. From the next packet onwards (segment number $S2$), the provider sends data with only the new ACKer's ID.

We realize that for packets with segment number between $S1$ and $S2$, the new ACKer's ACKs are not reliable since during that period, the new ACKer can miss packets because it is using the follower logic. Receiving an
ACK from the new ACker for $S2$ ($t3$ in the figure) might also not indicate the end of the shift since the original ACKer might have a longer latency than the new one. To better control the provider window during this phase, we assign every packet an ACKer. For packets in range $[S1, S2)$, although both ACKers might receive and send an ACK, we only consider the original ACKer. The new ACKer's ACKs in that range will be discarded by the provider. For packets with segment number $\geq S2$, the provider will use the new ACKer.

}















% Removed the router-assisted part
\hide{

%Since the sending rate might also be application specific, \eg, audio/video streaming, we leave the rate choosing as an end-to-end behavior. This kind of design also helps reduce the states kept in the routers and increases the scalability of the solution. Here, we only provide one kind of the rate control mechanism that can satisfy general-purpose data transmissions. But the architecture is not limited to the solution. And for scalability (\ie, a flow having more than $10^6$ consumers), we also provide a router-assisted mechanism to help with information collection.



\subsection{Router-assisted ACKer Selection}

Sending all the periodical feedback towards the data provider might not be scalable enough. In a large scale dissemination where the number of receivers comes to $10^6$ or more, it is very difficult for the data provider to process such large amount of data and the solution might also incur heavy load in the network. To reduce the data collection workload, we provide a general router-assisted aggregation model. We call it general because the model is not limited to congestion control, it can be used in any communication that needs aggregation to reduce workload, \eg, sensor network, \etc.

\subsubsection{Histogram-based aggregation}

Like basic ACKer selection, the histogram-based aggregation also requires the data collector to trigger a collection phase. He needs to define: 1) requirement of the responder, 2) how many cells are there in the histogram, 3) how to calculate which cell a responder belongs to, and 4) what's the timeout for collection period.

This message will be published using COPSS and when it is disseminated to the routers, the routers create an entry to aggregate data.
When a responder (a receiver in the flow) receives the message, if he meets the requirement specified by the message, he calculates the cell he is in and responds with the cell ID.
After collecting the responses from all the outgoing links or when the timeout reaches, a router sends the aggregated data upstream. Note that the routers here don't have to understand the meaning of the histogram, just forward the list of cell ID and count upstream.

The calculation of timeout might be a difficult part in the aggregation method. The optimal case would be the routers can estimate the time span on every hop and reduce that value when disseminating to the next hop. But the value is difficult to measure due to the effect of queuing. For simplicity, we assume that every router reduces a constant value before it sends the aggregation request downstream, say $2ms$. But it can be optimized by RTT measurement mechanisms like \jnote{try to cite some}.

\subsubsection{Use of aggregation in congestion control}

Now, the data provider sends an aggregation collection message to all the receivers instead of the original control message. Normally when a periodical feedback request starts, the responder range is all the receivers. He also needs to specify the cells. Here, the cells are calculated by the receive rate, duplicate rate, and mark rate. Since the maximum receive rate is limited by the sending rate, the provider can specify cells according to that value.

After the timeout period, the data provider can receive a histogram that indicates the distribution of receive rate among all the data receivers. If the distribution is clear enough to identify the cell the ACKer is in, the data provider indicates that all the receivers in that cell should respond with their own ID. Then, the data provider selects the first responder as the ACKer.

If the distribution is not clear enough, \ie there are too many receivers in the cell the ACKer should be in, the data provider should initiate another histogram collection phase, in which only the receivers in that cell should respond. And he provides a fine-grained histogram. He keeps doing this until when the distribution is good enough to pick an ACKer. \jnote{Do we need to prove the upper bound of the selection phase?}
}



==> implreceiver.tex <==
\section{Implementation of Receiver Window Control}
\label{sec-appendix-receivewindowcontrol}
\subsection{Network support for MPR delivery}
To control the congestion window size on the receiver side as we described in \S\ref{sec-congestioncontrol-receivers}, \name needs the cooperation from the network.
The intermediate routers need to piggyback the instantaneous PR with the data packets similar to REM.
The PR is the current value of the counter we added in PIT to accumulate such ``any-next'' requests.

In order to allow the receivers get minimum PR (MPR) in the whole path, we add an MPR field in the data packet.
Data provider should initiate this field as $+\infty$.
The intermediate routers forward the packet based on PIT and sets MPR$\leftarrow$$min($MPR$,$PR$)$.
Note that the PR here is PIT count for the flow \emph{towards the interface} of the the data packet.
If the router needs to replicate the data packet, the MPR on each packet might be different.
To ensure the integrity of MPR (if necessary), the intermediate routers (and the data provider) can sign the MPR separately without touching the content of the packet. The intermediate routers can use the private key of the ISP and the receivers can check the signature via the ISP's public key.

For a receiver ($C$), the minimum instantaneous PR always appears on the branching point of $C$ ($Br(C)$).
According to the definition, on the router $Br(C)$, there exists other outgoing face(s) that can receive faster than $C$, or it is the \first hop router of the data provider if the $C$ can receive at a rate faster than the sending rate.
In Fig.\ref{fig:topology2}, $Br(C_1)$$=$$R_3$ since $R_3$ has subtree $R_8$ that can receive at $2Mbps$. Likewise, $Br(C_2)$$=$$R_1$.
The routers below $Br(C)$ might see fresh requests sent from $C$ and their PR value should always $\ge$ the PR at $Br(C)$;
The routers above $Br(C)$ would see more pending requests from another interface and therefore the value should be $\ge$ the PR at $Br(C)$ also.

%In other words, each receiver is the fastest in the subtree under its branching point and this controls the request rate of that subtree.

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/StateMachineMinPS}
    \vspace{-1mm}
    \caption{State machine for receiver window increase}
    \vspace{-5mm}
    \label{fig:window}
\end{figure}




%When the intermediate router forwards the packet, it looks up its own pending request count on that face $PR_r$ and set .
%overwrites the packet count if it is  smaller.
%Every receiver records the MPR and decides whether to increase the window size based on the minimum MPR observed in the window (MMPR).
\subsection{Receiver decision based on the MPR}
On receiving the data packets with the instantaneous MPR value, the receiver picks the smallest one in a window (MMPR).
Our mechanism uses a state machine (Fig.~\ref{fig:window}) to keep track of how long the MMPR on a receiver is in a particular state ($=$$0$, $<$$X$, or $>$$X$) and decide the size of the next window. $X$ is a parameter that decides the maximum number of pending requests that are used to absorb a burst. We found $X$=$5$ works well across different evaluations we performed.
The receivers adjust their congestion window based on the following rules:
%Window behavior based on MMPR is as follows:

\begin{enumerate}
\item Every receiver starts in the ``Grow'' state ($G$) and stays in $G$ as long as MMPR$=$$0$.
MMPR$=$$0$ means the data from the provider can always consume all the pending requests, and therefore the receiver should increase the window size.

\item Whenever MMPR grows above $X$, the receiver should stop increasing the window immediately.

\item \label{enu:windowrule-rem}
    On seeing an REM, no matter which state it is in,  a receiver should clear all the MMPR counters, reduce the window size by half (multiplicative decrease) and go to $G$ (not shown in Fig.~\ref{fig:window}).

\item MMPR can fluctuate even when the window size is large enough due to a short burst of packets from the provider. We therefore define the Stable state ($S$) as the receiver sees  MMPR$>$$0$ for more than $Y$ windows. %\jnote{instead of defining stable state is $>X$ for $Y$ windows.}
Window should stop increasing in state $S$.
%$Y$ is another parameter we will discuss later.

\item To count $Y$ windows, we introduce an intermediate Counting state ($C$). While in state $C$, the receiver keeps increasing the window until the count $Y$ is reached (to $S$) or the MMPR grows larger than $X$ (to $P$).

\item When the MMPR drops to 0 in $S$, it might indicate that one of the two conflicting scenarios is happening: either the publisher increases the sending rate and thereby consumes the pending requests, or there is a competitor on the bottleneck that causes the receiver to send requests slower. The receiver should increase the window in the first case while decrease it in the second. We choose to wait for $Y$ windows before increasing the window. If a competitor shows up, the receiver should see marks and operate based on rule~\ref{enu:windowrule-rem}.

\end{enumerate}

The parameter $Y$ reflects the stability of the mechanism. A larger $Y$ means the longer a receiver waits on seeing MMPR $=0$, it can be beneficial in the presence of a competitor, but will under-utilize the network when the provider increases the sending rate. We set $Y$$=$$X$$=$$5$ in implementation.
The state transitions for the example in \S\ref{sec-congestioncontrol-receivers} is also shown in Fig.~\ref{fig:resultwindow}.
%\knote{all of this is too complicated and we are not abstracting the idea to a level that is easy to understand. The reader is left with a view that the mechanism is built up as we went along, filling in the holes we discovered. We need a better way to abstract it and elevate the writing, and put all the detail possibly in an algorithm in the appendix.}


==> mpr_-_Copy.tex <==
\subsection{Handling Additive Increase}
\label{sec-congestioncontrol-receivers}
% Mayutan: should we use source or sender instead of publisher? Lets use provider as done in other parts

\hide{
The multiplicative decrease on seeing REM can work well in the presence of competing flows, but a simple additive increase mechanism is not sufficient when the path to the receiver has high bandwidth.
Unlike TCP or ICP, the transmission rate on the provider is not controlled by the receivers' congestion windows.
The receivers with available bandwidth (or a fair share on a multiplexed link)
higher than the transmission rate will not see any marks and their window will continue to grow to a highly inflated value (especially if there is no limit).
This growth in the window essentially causes a large number of pending requests to be queued at the upstream router.
These pending requests will allow a large number of packets to be delivered in a burst towards the receiver when the provider decides to increase the transmission rate or new contention occurs on the path.
The large build up of a queue at the bottleneck router also increases the feedback delay.
Thus, for the period when a burst of packets is transmitted from a buffer that has high occupancy, those packets will be marked,
% since they receive an unfair share of the available bandwidth,
thus causing the receiver to react aggressively and reduce the window. This form of ``bang-bang'' effect has the potential to under-utilize the network or cause unfairness between flows over a
subsequent interval.
}

%Although all the receivers have the same need -- control the pending requests it sends,
The optimal window size can vary from receiver to receiver and even from time to time on a single receiver due to different bandwidth-delay-products (BDPs).
We therefore propose a dynamic process on each receiver that tries to keep the window size close to the optimal value.
The core of the process is based on constantly observing and reacting to the instantaneous minimum pending request count (MPR) on the path.

The network piggybacks the instantaneous MPR while data packets are forwarded towards the receivers.
Note that different receivers can see different MPR even for the same data packet since MPR appears at the branching point (the router having other outgoing faces that are receiving faster than the current receiver).
A receiver should observe all MPRs in a window and ensure:
%Our solution is therefore tailored for each receiver to decide on its window increase based on an observation over a period of time of the instantaneous minimum pending request count (MPR) on the path.
\begin{inparaenum}[\itshape 1\upshape)]
\item these values are as small as possible (to avoid too many pending requests in the path),
\item the minimum MPR (MMPR) is larger than a small value (to avoid all the pending requests consumed by future short burst), and
\item glitches are filtered.
\end{inparaenum}
To simplify the calculation, our mechanism decides on the window increase on MMPR alone. It will stop increasing the window when MMPR is larger than $X$ and only increase window when it can rule out the possibility of reacting to a transient (based on the state machine depicted in Fig.~\ref{fig:window} , see~\cite{TechReport} for the detailed algorithm).



%Because of the above considerations,
%We seek to limit the window size for the receivers with a bottleneck bandwidth larger than the publication rate.
\hide{
\subsubsection{Obtaining MPR}
The network piggybacks the instantaneous MPR while data packets are forwarded towards the receivers.
Data providers initiate the MPR field in the packet to $+\infty$, and the intermediate routers that forward the packet based on the PIT set MPR$\leftarrow$$min($MPR$,$PR$)$.
Note that the PR here is the PIT count for the flow \emph{towards the interface} of the the data packet.
If the router needs to replicate the data packet, the MPR on each packet might be different.
}
\hide{
\subsubsection{Receiver Behaviour}

\hide{
Therefore, while deciding if the receiver should increase the window, our mechanism needs to avoid:
\begin{inparaenum}[\itshape 1\upshape)]
\item too many pending requests in the path,
\item all the pending requests consumed by a short burst, and
\item unnecessary increase due to transient changes.
\end{inparaenum}
}

Different receivers could see different MPR even for the same data packet since MPR appears at the branching point (the router having other outgoing faces that are receiving faster than the current receiver). For a receiver ($C$), the minimum instantaneous PR always appears on the branching point of $C$ ($Br(C)$).
According to the definition, on the router $Br(C)$, there exists other outgoing face(s) that can receive faster than $C$, or it is the \first hop router of the data provider if the $C$ can receive at a rate faster than the sending rate.
In Fig.\ref{fig:topology2}, $Br(C_{11})$$=$$R_1$ since $R_1$ has subtree $R_4$ that can receive at $2Mbps$. Likewise, $Br(C_{21})$$=$$R_0$.
The routers below $Br(C)$ might see fresh requests sent from $C$ and their PR value should always $\ge$ the PR at $Br(C)$;
The routers above $Br(C)$ would see more pending requests from another interface and therefore the value should be $\ge$ the PR at $Br(C)$ also.
}
%To simplify the calculation, our mechanism decides on the window increase on MMPR alone. It will stop increasing the window when MMPR is larger than $X$ and only increase the window when it can rule out the possibility of reacting to a transient.

%\subsubsection{Reacting to MPR}


We use an example to trace the MMPR and the window increase decisions to aid in understanding how the scheme works ($X$ is set to 5 in the example).
%Fig.~\ref{fig:window} presents a state machine based representation of how the state of the receiver window varies according to the MMPR.
We use an example to trace the MMPR and the window increase decisions to aid in understanding the scheme.
%The MPR, window size and the state transitions in Fig.~\ref{fig:resultwindow} are shown for a receiver with $2Mbps$ available bandwidth.
Every cross represents a decision made at the end of a window.
The MMPR grows with the window size after $1 sec$. 4 windows later, the MMPR reaches 5 and the receiver stops increasing the window.
The MMPR stays at around 5.
Although the MMPR becomes lower than 5 for several windows at around $4 sec$ (due to the transient changes) the window size is not increased.
When there is new contention at the bottleneck link (additional competing flow) occurring between $10 sec$ and $25 sec$, MMPR drops to 0 and the receiver then
starts to increase the window.
The receiver receives packets marked as a result of REM at $12 sec$ and then to perform normal AIMD to respond to the
contention introduced by the competing flow.
%At $10s$, a competitor shows up on the bottleneck link and the MPR drops to 0. But the receiver maintains the window size for 5 windows before increasing. The seemingly wrong decision occurs because it takes time for the moving average to increase on the bottleneck router.
%When the competitor re-appears for a second time at $25s$, we do not observe an increase in the window size.
We show how this mechanism aids in achieving fairness in \S\ref{sec-eval-emulationfairness} and \S\ref{sec-eval-receiverlogic}.

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/StateMachineMinPS}
    \vspace{-3mm}
    \caption{State machine for receiver window increase}
    \vspace{-7mm}
    \label{fig:window}
\end{figure}

\hide{
\subsection{Implementing  Receiver Window Control}
\subsubsection{Network support for MPR delivery}

\mnote{Moved parts of it above}

To control the congestion window size on the receiver side as we described in \S\ref{sec-congestioncontrol-receivers}, \name needs the cooperation from the network.
The intermediate routers need to piggyback the instantaneous PR with the data packets similar to REM.
The PR is the current value of the counter we added in PIT to accumulate such ``any-next'' requests.


In order to allow the receivers get minimum PR (MPR) in the whole path, we add an MPR field in the data packet.
Data provider should initiate this field as $+\infty$.
The intermediate routers forward the packet based on PIT and sets MPR$\leftarrow$$min($MPR$,$PR$)$.
Note that the PR here is PIT count for the flow \emph{towards the interface} of the the data packet.
If the router needs to replicate the data packet, the MPR on each packet might be different.

To ensure the integrity of MPR (if necessary), the intermediate routers (and the data provider) can sign the MPR separately without touching the content of the packet. The intermediate routers can use the private key of the ISP and the receivers can check the signature via the ISP's public key.

For a receiver ($C$), the minimum instantaneous PR always appears on the branching point of $C$ ($Br(C)$).
According to the definition, on the router $Br(C)$, there exists other outgoing face(s) that can receive faster than $C$, or it is the \first hop router of the data provider if the $C$ can receive at a rate faster than the sending rate.
In Fig.\ref{fig:topology2}, $Br(C_{11})$$=$$R_1$ since $R_1$ has subtree $R_4$ that can receive at $2Mbps$. Likewise, $Br(C_{21})$$=$$R_0$.
The routers below $Br(C)$ might see fresh requests sent from $C$ and their PR value should always $\ge$ the PR at $Br(C)$;
The routers above $Br(C)$ would see more pending requests from another interface and therefore the value should be $\ge$ the PR at $Br(C)$ also.

}

%In other words, each receiver is the fastest in the subtree under its branching point and this controls the request rate of that subtree.





%When the intermediate router forwards the packet, it looks up its own pending request count on that face $PR_r$ and set .
%overwrites the packet count if it is  smaller.
%Every receiver records the MPR and decides whether to increase the window size based on the minimum MPR observed in the window (MMPR).
\hide{

\subsubsection{Receiver decision based on the MPR}
On receiving the data packets with the instantaneous MPR value, the receiver picks the smallest one in a window (MMPR).
Our mechanism uses a state machine (Fig.~\ref{fig:window}) to keep track of how long the MMPR on a receiver is in a particular state ($=$$0$, $<$$X$, or $>$$X$) and decide the size of the next window. $X$ is a parameter that decides the maximum number of pending requests that are used to absorb a burst. We found $X$=$5$ works well across different evaluations we performed.
The receivers adjust their congestion window based on the following rules:
%Window behavior based on MMPR is as follows:

\begin{enumerate}
\item Every receiver starts in the ``Grow'' state ($G$) and stays in $G$ as long as MMPR$=$$0$.
MMPR$=$$0$ means the data from the provider can always consume all the pending requests, and therefore the receiver should increase the window size.

\item Whenever MMPR grows above $X$, the receiver should stop increasing the window immediately.

\item \label{enu:windowrule-rem}
    On seeing an REM, no matter which state it is in,  a receiver should clear all the MMPR counters, reduce the window size by half (multiplicative decrease) and go to $G$ (not shown in Fig.~\ref{fig:window}).

\item MMPR can fluctuate even when the window size is large enough due to a short burst of packets from the provider. We therefore define the Stable state ($S$) as the receiver sees  MMPR$>$$0$ for more than $Y$ windows. %\jnote{instead of defining stable state is $>X$ for $Y$ windows.}
Window should stop increasing in state $S$.
%$Y$ is another parameter we will discuss later.

\item To count $Y$ windows, we introduce an intermediate Counting state ($C$). While in state $C$, the receiver keeps increasing the window until the count $Y$ is reached (to $S$) or the MMPR grows larger than $X$ (to $P$).

\item When the MMPR drops to 0 in $S$, it might indicate that one of the two conflicting scenarios is happening: either the publisher increases the sending rate and thereby consumes the pending requests, or there is a competitor on the bottleneck that causes the receiver to send requests slower. The receiver should increase the window in the first case while decrease it in the second. We choose to wait for $Y$ windows before increasing the window. If a competitor shows up, the receiver should see marks and operate based on rule~\ref{enu:windowrule-rem}.

\end{enumerate}

The parameter $Y$ reflects the stability of the mechanism. A larger $Y$ means the longer a receiver waits on seeing MMPR $=0$, it can be beneficial in the presence of a competitor, but will under-utilize the network when the provider increases the sending rate. We set $Y$$=$$X$$=$$5$ in implementation.
%The state transitions for the example in \S\ref{sec-congestioncontrol-receivers} is also shown in Fig.~\ref{fig:resultwindow}.

%\begin{figure*}[t!]
%\vspace{-3mm}
%\centering
%\begin{minipage}[b]{0.7\linewidth}\centering%
%\input{figures/ResultStateMachine.tex}\vspace{-3mm}%
%\caption{Result of window control at the receiver using state machine}%
%\label{fig:resultwindow}%
%\end{minipage}\hspace{-0.01\linewidth}%
%\begin{minipage}[b]{0.3\linewidth}\centering%
%\input{figures/LocalFIBPropagation2.tex}\vspace{-2mm}%
%\caption{Example of different kinds of repair}%
%\label{fig:localrepair}%
%\end{minipage}
%\vspace{-6mm}
%\end{figure*}

}
\hide{
\knote{This transition is NOT clear. You just suggested that AIMD was great in the previous subsection. Now you say it is not sufficient. You haven't yet made the case for it! What is an ACKer? You have not described that either. You have not yet talked about how to deal with heterogeneous receivers. Below is an attempt.}
While the simple case of receivers having the same bottleneck bandwidth
from the publisher can be fairly managed with the use of REM and an AIMD policy for controlling the window, it is not as effective in the heterogeneous case.
This is especially true when we seek to have the publisher's rate go beyond the
slowest receiver's rate. Based on the application need, we may choose to have
the publisher send at the rate of the majority of the receivers (the median rate) or that of the receiver whose rate is in the top quartile etc., and then depending on repair to accommodate the other receivers. We introduce the notion
of an 'ACKer', which is the designated receiver whose average receive
rate matches this application need. The 'ACKer' generates new requests for
data packets as it receives and consumes what has been sent by the publisher.
Thus, it controls the publisher's rate. While the other receivers also adjust their
window size based on REM marking, they do not affect the publisher's rate.
While the problem of choosing the ACKer is
a complex one, we solve it in a subsequent section. For now, assuming that
the ACKer has been chosen correctly, we examine the window management
policy for
those receivers that are not ACKers.
\mnote{I think that the case fo heterogenous receivers needs to be made in the overall architecture and here we should focus on only CC and probably remind the readers of the issue in one line. We can probably move some of the above lines to overall-arch}
}


\hide{

The consequence of such a growth could be severe since %, especially because in this one-to-many scenario,
the changes in the receiver's window cannot affect the source's sending rate. \knote{not clear what you mean by this. So, if it
doesn't affect the source's rate what does it do by growing to a large value? Do you mean: even though it doesn't change
the original publisher's sending rate, it allows a large number of packets to be delivered in a burst towards the receiver. This
burst has the consequence of over-running the bottleneck in the path towards the receiver, thus impacting not only this receiver,
but others? Please re-write as stated.}
One possible consequence is when the publisher decides to increase the publication rate, the large window will cause a burst of packets to arrive at the bottleneck router towards that receiver.
%Packets will potentially be queued at that router.
% Failure will happen when the window is too large because of the delayed control.
%Say, an endhost has 1000 pending requests, and suddenly upstream sends 1000 packets, all the packets will be queued, and many of them are marked.
%The end host will now resend the requests and on seeing marks, he will reduce window. The solution for ¡°reduce window only once in one window¡± will not work since 1000 packets can represent many windows. Therefore, the rate of the endhost is dramatically reduced after this 1000 packets, and for a very long time. And during this 1000 packets (or even more), the receiver will get an unfair shar.
%This is why we need to avoid the window growing too large. Need to mention it somewhere.
It also has the consequence that the large build up of a queue at the bottleneck router increases the feedback delay.
Thus, for a period of time when the burst is transmitted, those packets will be marked as they receive an unfair share
of the available bandwidth, thus causing the receiver to react and reduce the window. This form of 'bang-bang' effect has the potential to under-utilize the network over a subsequent interval.
While an excessively large window might cause inefficiency and unfairness, a very  small window might also lead to inefficiency because a short burst caused by transient congestion might consume all the pending requests and result in unnecessary packet loss.


%These packets will be buffered on the bottleneck router and cause delayed control effect.
%During a period of time, the receiver will receive an unfair share (all of the available bandwidth) and reduce the window size to very small value since many of these packets may carry marks, resulting in an under-utilization of the network in the next period.
%
%
%The large number of packets buffered at the router essentially serves these requests.
%Moreover, as with traditional window based protocols with a flow having an inappropriately large window, the AIMD based decrease of the window will still take some time to reduce to a fair value starting from this inflated value.
%This results in unfairness and/or inefficiency issues.% and maintaining a proper window size is critical.% for good network resource usage.
%This is due to the fact that the receiver (even with window size = 1) sends a request on receiving data and is served data from the packets existing in the queue.
%Feel it is still not clear... I'm mainly talking about all the data packets are in the queue, and the receiver sends out a request on seeing a data and he will receive at the bottleneck rate. % Mayutan: agree, we need to further improve this para. Moreover, I need to discuss with you if the term bottleneck rate is right when window size = 1.
%This will cause extreme unfairness if other flows are sharing the same link. The second consequence could be that when a new (set of) flows arrive at the bottleneck, the AIMD mechanism will take longer to arrive at a fair value from this artifically inflated window size.
%\looseness-1
}


\hide{ % Not needed
The following questions arise: 1) How to decide whether a receiver has sufficient bandwidth? % to sustain the flow
%If the receiver's bandwidth is large enough, we need to limit the receiver's window; otherwise we should allow the window to continue to increase until it sees marks from the routers.
This determines \emph{if} the receiver is going to increase the window.
2) \emph{How large} should the maximum window be? Due to the differing bandwidth-delay-products (BDPs), different receivers will need different window sizes.
3) \emph{When} to increase the window? The window size depends on the contention seen from other flows.
%\looseness=-1
%It is very difficult for end-hosts to control their window without knowing the state in the network including the available bandwidth and the presence of competitors.
}

\hide{
We observe that the purpose of controlling the receiver's window size is %primarily
to control the number of \emph{pending requests} at the routers, especially the router at a branching point in the path.
% define branching point
The branching point of a receiver is the router having other outgoing faces that can receive faster than this receiver, or the \first hop router of the data provider if the receiver can receive at a rate faster than the sending rate.
In Fig.\ref{fig:topology3}, the branching point of $C_1$ is $R_3$ since $R_3$ has another outgoing face that can receive at $2Mbps$. Likewise, the branching point of $C_2$ is $R_1$.
In other words, each receiver is the fastest in the subtree under its branching point and this controls the request rate of that subtree.


% MPR
We observed that, because of feedback delay, different routers on the path see different PR values, but the branching point (no matter where it is on the path) always has the minimum value among them (MPR).
This is because the routers below the branching point might see new pending requests sent from the receiver and their PR value should always $\ge$ the PR at the branching point;
The routers above the branching point would see more requests from another interface and therefore the value should be $\ge$ the PR on the branching point also.




Our mechanism tries to control this MPR (by controlling the congestion window on the receiver) when there is no congestion indication (REM). %\knote{ what congestion indication? from where?}
The MPR should be always larger than 0 to ensure the receiver can receive every packet from upstream, but not too large to cause significant feedback delay.
We also noticed that MPR changes constantly and it only reflects the instantaneous path state in the recent past.
Therefore, we use the minimum MPR observed in a window (MMPR) to decide if the receiver should increase congestion window.
In brief, if MMPR $\le X$ ($X$ is a small number), the receiver should increase window to absorb a possible burst, otherwise the receiver should maintain the current window size. \knote{what is the motivation for this mechanism, and how do you abstract what it achieves. Too much detail, no abstract description of the concept.}\jnote{OK. Will rewrite}
}

%However, we discovered that the Minimum Pending Request (MPR) value on the routers up the tree (the path from the provider to the receiver) is the most relevant, as that limits the burst flowing down to the bottleneck link.
%If the MPR becomes too large, a burst of arrivals might occur and fill up the queue. If the MPR becomes too small, the pending requests will be consumed by the data packet before new requests arrive and thus cause the underutilization of the bandwidth.
%\jnote{Want to remove the following 2 sentences, meaningless if we don't go into the detail, and anyway you have can never know where is the branching point}
%/mnote{agree}
%However, note that the MPR always appear at the \textit{branching point} towards this receiver.
%The branching point is the router having other outgoing faces that can receive faster than this receiver, or the \first hop router of the data provider if the receiver is faster than the publication rate.


\hide{
We use an example to trace the transitions in the state machine to aid in understanding. how the scheme works
The MPR, window size and the state in Fig.~\ref{fig:resultwindow} are shown for a receiver with $2Mbps$ available bandwidth.
The MMPR grows with the window size after $1 sec$, and the receiver shifts to state $C$. 4 windows later, the MMPR reaches 5. The receiver enters state $P$ and stops increasing the window.
At the end of the $5^{th}$ window, the receiver enters state $S$ and the MMPR stays at around 5.
Although the MMPR becomes lower than 5 for several windows at around $4 sec$ they are seen as the false alarm \knote{how??} and the window size is not increased. The MMPR later shows this was the right decision \knote{how is this achieved?}.
%
When a competitor arrives at the bottleneck link between at $10 sec$ and $25 sec$, MMPR drops to 0 and the receiver behaves as we expected.
%At $10s$, a competitor shows up on the bottleneck link and the MPR drops to 0. But the receiver maintains the window size for 5 windows before increasing. The seemingly wrong decision occurs because it takes time for the moving average to increase on the bottleneck router.
%When the competitor re-appears for a second time at $25s$, we do not observe an increase in the window size.
We show the intra- and inter-protocol fairness in \S\ref{sec-eval-receiverlogic}.%\looseness-1
\knote{what is inter and intra protocol? What do you mean??}
}


%\mnote{Can we refer to the state machine while talking about rules too, e.g. we call it entered stable state $S$ and so on. }
%\jnote{I think this part is about the rules, or reasoning, state machine is an implementation. That's why I separate them.}
%\mnote{change the itemize to reduce white space on the left}
%\mnote{where is X, Y defined or shown? or how does a receiver determine $X$ in order to stop increasing}
%\begin{itemize}
%\item If the MPR in the current window is larger than $X$, stop increasing the window immediately. This is the basic rule to avoid the MPR from becoming too large.
%\item If the MPR is larger than 0 for $Y$ windows (we think of it as having entered the stable state), even if the MPR in the current window is smaller than $X$ (but still larger than 0), the receiver should not increase the window. This rule is set to prevent fluctuations.
%We observed that due to the variability in the network, this behavior may occur for a window or two, where the MPR might be smaller than $X$. If we increase the window size in that situation, MPR in the next window may grow larger than $X$.
%\item In the stable state, when the MPR in the window is dropped to 0, the receiver will wait for $Y$ windows before increasing the window size. MPR might drop to 0 for two reasons: one is the provider increases his sending rate and consumes the pending interest; the other is a competitor appears on the bottleneck link.
%In the first scenario, the receiver should increase the receive window.
%It is easy to understand the first reason, more data packets arrive and thereby consume the pending subscriptions.
%When the provider increases his sending rate, the receiver should increase the receive window.
%In the scenario where a competitor just appears, the receiver receives data packets slower than before and also sends requests slower.
%The pending subscriptions will get consumed for a short period. But in such a scenario, the data provider should reduce the window size (e.g., by half in TCP) rather than increase it. Since there is no way for a receiver to know what is the cause of dropping to 0 and he needs to make conflicting decisions for these two scenarios, we let the receiver pause for several windows before starting to increase it.
%\item Whenever a receiver receives a data packet with an REM mark, the receiver will reduce the window size by half, clear all the counters and then subsequently seek to find the right window size by gradually growing the window size using the AIMD policy.  %\knote{CONFUSING. You say reduce the window. Then you say grow the window. Confusing.} \mnote{fixed}
%\end{itemize}

%We use a state machine (shown in Fig.~\ref{fig:window}) to keep track of how long the subscriber is in a particular
%state (say, minimum MPR in the window is equal to 0, smaller than $X$, or larger than $X$).
%To make the state machine cleaner, we didn't put rule 4 in the figure. In the real implementation,
%All the states have a transition to $G$ on receiving a mark (not shown in Fig.)
%We use an example to trace the transitions in the state at the receiver to aid in understanding. Let both $X$ and $Y$ be initally set to 5.
% to show a walk through of how the state changes on the receiver.

%At the beginning, the receiver starts with the $Grow$ ($G$) state and stays in $G$ whenever the minimum MPR in the window is 0 (the first second). The MPR grows with the window size after $1s$, and the receiver shifts to $Count$ ($C$) state. While staying at $C$, the receiver still increases the window size. But after 4 windows, the minimum MPR in the window reaches 5, so the state becomes
%$Pause$ ($P$), and the window stops increasing. At the end of that window, there has already been 5 windows with MPR larger than 0, so the receiver goes to $Stable$ ($S$) state and the minimum MPR stays at 5. We can also see that the MPR becomes lower than 5 for several windows around $4s$. But we don't increase the window size based on the second rule above. This is
%the right reaction as otherwise the window might increase several times unnecessarily.

%At $10s$, we introduce a competitor on the bottleneck link. The MPR then drops to 0 as we described above. But the receiver maintains the window size for 5 windows before increasing. The seemingly wrong decision occurs because it takes time for the moving average to increase on the bottleneck router.
%When the competitor re-appears for a second time at $25s$, we do not observe an increase in the window size.%\knote{???}\mnote{modified it}
%But we decide not to increase the observation period before we increase the window size because the decision will also affect the time a receiver waits when a publisher increases the sending rate.

%During the period the competitor exists, there are several windows with MPR larger than 0 (but smaller than 5), the receiver enters $Count$ state but still increases the window. It returns to $Grow$ state almost immediately after that.
% These fluctuations are smoothed out with our state machine.
%The state machine also helps remove fluctuations that can be observed in Fig.~\ref{fig:resultwindow}. We also see that the receivers share the bandwidth fairly and the rate converges fast. The receive rate figure is omitted due to the space limitation.



\hide{
\begin{enumerate}
\item Why not router-base fair queuing? 1) Complexity, 2) Sally Floyd's topology

\item Assume pub send at a certain rate (or align to a certain ACKer, based on the decision), separate majority and minority

\item Minority per-packet subscription

\item Shift between Majority and Minority. TODO: need to decide how to shift

\item Network friendliness

\begin{enumerate}
\item Minority \vs Minority : fair

\item Minority \vs Majority: Majority will turn to minority. 1) If Majority has more than its fair share, it will drop to the fair share; 2) If Majority doesn't have its fair share, it will stay close to the publication rate.

\item Majority \vs Majority : 1) having enough bandwidth, no problem; 2) don't have enough bandwidth: both go to minority and keep either a. fair share or b. one receive at pub rate and the other receive the remaining rate.

\item Minority \vs ACKer: fair

\item ACKer \vs ACKer: fair

\item Majority \vs ACKer: same as Majority \vs Minority

\end{enumerate}

\item Overall Performance
\begin{enumerate}
\item Sally Floyd topology
\item 8-sub topology with 2 flows
\end{enumerate}

\end{enumerate}
}

%\begin{figure}[t!]
%    \centering
%    \includegraphics[width=0.44\textwidth]{figures/StateMachineMinPS}
%    \input{figures/StateMachineMinPS.tex}
%    \caption{State machine for follower window increase}
%    \label{fig:window}
%\end{figure}


==> proof.tex <==
\section{Proof of Theorem \ref{theorem-outofsyncrequirement}}
\label{sec-appendix-proof-theorem}
\vspace{-1mm}



==> pubcontrol.tex <==
The data-provider's sending rate is typically determined by application requirements.
%Different applications have different requirements on the sending rate at the data-provider.
Applications like audio/video streaming need a certain minimum rate for proper audio/video progression and might also have a limit on the maximum rate. However, certain other applications such as file delivery are more elastic and therefore the sender can find a balance between the average completion time and the network load (as illustrated in Fig.~\ref{fig:repair_throughput}).
\hide{
% Mayu: can add if space is available
Even if the application chooses a sending rate that is higher than all the receivers' bandwidth, it will not result in a congestion collapse. This is due to the fact that the packet will be ``dropped'' at the $1^{st}$ hop router of the data provider since the pending requests are consumed faster than their accumulation at that router.
}

%From Fig.~\ref{fig:repair_throughput}, we can see that if the sending rate is too low, the flow under-utilizes the network. Although the network load is low, the average completion time can be quite high. But when the sending rate becomes too high, a large portion of the data will have to be retransmitted by repair. The retransmission load becomes high and the average completion time might further increase if the repair causes congestion in the network.
%Since there are differences in the desired level of control over the sending rate from different applications, we believe it is appropriate to design it at the application layer (or at least allow applications to specify their desired level of control).
%For applications with a specific required rate, the data provider only needs to send the packets at that constant rate.
%The absence of pending requests at the $1^{st}$ hop router will result in transmission not making progress.
%Therefore, no matter how fast the data provider can send the data, the data will not cause congestion collapse in the network.

For general-purpose data transmission, we suggest the data provider send at the rate that the \emph{majority} of the receivers can receive. Therefore, those consumers can receive all of the data transmitted without much repair, % (or only repair a small part)
while the slower receivers (the \emph{minority}) will depend on the other receivers % (especially the majority)
for the missing packets.
However, the estimation of the receive rate of the majority is not easy either, because of the highly dynamic nature of network.
Therefore, instead of \emph{estimating} the receive rate for the majority directly,
we divide the task into two parts: 1) find a proper receiver (normally the slowest in the majority) as an \emph{ACKer} and 2) \emph{align} the content provider's sending rate to the ACKer's available bandwidth.
%This solution is similar to pgmcc\cite{pgmcc}.
Unlike pgmcc\cite{pgmcc}, the ACKer we pick is the slowest in the majority, not the slowest among \emph {all} the receivers.
This allows our solution be more efficient than pgmcc because we exploit the efficient repair capability in ICN.
Note that our solution can also align to the slowest receiver if the application demands it, but by having the ability to also align to a constant rate or to that of the majority, our solution is more flexible and can support different types of applications needs. % (see \S~\ref{sec-discussion}).

%\subsection{ACKer Selection}

A critical component of the mechanism is the selection of the
ACKer.
Due to the dynamic nature of the network, the slowest receiver in the majority might change from time to time.
Therefore, the provider should have the ability to change the ACKer based on network conditions.
But compared to the per-RTT estimation of sending rate, the ACKer selection can be made over a relatively longer time scale. The provider initiates the ACKer selection periodically.

\hide{
\subsubsection{Initiation phase}
Unlike some of the IP multicast protocols, \name does not adopt a session-initiation phase.
The provider starts to collect data concurrently with data dissemination.
%Thus, the provider has no information of the current receivers for the first period.
Therefore, when sending the first packet, the provider indicates that each consumer should respond with his unique ID in the flow to the provider.
For the second packet, the provider uses the receiver that responds first as the ACKer, since in the worst case scenario, there may be only one receiver.
Later, as the provider receives more ACKs for the first packet, he can elect the ACKer based on the latency until the end of the initiation period.
}

%\subsubsection{Periodic feedback}
Unlike some of the IP multicast protocols, \name does not adopt a session-initiation phase.
Instead, it relies on feedback sent by the receivers to the first packet in order to elect the initial ACKer.
%On receiving data for a period of time, the receivers are able to collect throughput statistics.
Periodically, the data provider triggers the collection of receiver statistics, by
% To reliably deliver the trigger information, we
piggy-backing a trigger packet containing the statistics collection range (start segment ID and end segment ID) for a period of time (\eg, a window).

%Multiple values need to be used to get the estimate of the available bandwidth at the receiver.
%The first is the number of packets received. This is a direct value to estimate the current receive rate.
The number of packets received can be used to estimate the current receive rate.
But receivers with an available bandwidth higher than the ACKer will all have the same receive count.
Therefore, we depend on  a second value: the number of received packets that were marked.
Faster receivers will receive fewer marked packets compared to the ACKer.
Different receivers might have received a slightly different number of packets, due to queueing at routers.
To better reflect the receive rate, we also take the last received packet into consideration.
%On receiving a statistics collection packet with a 'start' and 'end' range, every receiver encapsulates the number of packets received, the number of packets marked and the segment ID of last received packet into an Interest packet. The Interest packet has the flow ID as the prefix and the network knows how to reach the data provider since the provider already advertized the FIB of the flow ID.
On receiving the statistics from the receivers, the provider calculates the score of every receiver as
\begin{equation}\label{equ-acker-selection}
  S=\frac{ReceivePktCount - 0.5 \times MarkPktCount}{LastReceiveID - RangeStart}.
\end{equation}
We value a marked packet a being half as good as a normal packet, so as to space out the faster receivers. The receiver at rank $R$ will be elected as the new ACKer.
However, we believe that changing the ACKer frequently might affect the stability of the flow
%(the RTT of the ACKer might change).
and therefore only elect a new ACKer if the current ACKer is not in the range $R \pm R_{th}$.
But when the condition in the network or the receivers changes dramatically, a shift on the ACKer is inevitable.
%\jnote{Is ACKer shift removed? Is that OK?}
%Then, the publisher would have to select either a different ACKer.

Selecting a slower ACKer than the current one is relatively easy. Using Eq.~(\ref{equ-acker-selection}), we can select a slower receiver that has a lower receive count and higher mark count in proportion to their available bandwidth.
But selecting a faster ACKer is not straightforward since the new ACKer should be among the faster receivers who all receive at the same rate as the current ACKer.
The mark count in Eq.~(\ref{equ-acker-selection}) will take effect in this case.
Although the faster receivers have the same receive count as the ACKer, they have a lower mark count.















\hide{
\subsubsection{Selecting a slower ACKer}
Often a competing flow appears on a link closer to the root of the dissemination tree and thus many receivers' rate is lowered. If the ACKer is among the affected receivers, the window-based solution would adjust the throughput automatically. But if the ACKer is not affected, the flow needs to find a slower ACKer in order to have the sending rate match the new majority and to avoid wastage of resources and time on the repair phase. The departure of fast receivers can also cause a provider to try to select a slower ACKer.

Selecting a slower ACKer is relatively easy. The slower receivers always have a lower receive count and higher mark count in proportion to their available bandwidth. Using equation~\ref{equ-acker-selection}, we easily find a proper new ACKer.


\subsubsection{Select a faster ACKer}

The provider might also have to elect a faster ACKer due to the departure of slower subscribers or on completion of a competing flow. But selecting a faster ACKer is not straightforward since the new ACKer should be among the faster receivers who all receive at the same rate as the current ACKer.
The mark count in equation~\ref{equ-acker-selection} will take effect in this case.
Although the faster receivers have the same receive count as the ACKer, they have a lower mark count. If two receivers have the same score, we will order the receivers based on their response time. The receiver with lower RTT (who responds faster) is ranked higher since he will have higher throughput.

This estimation might not be accurate. But if we analyse the election in the long run, the selection of an ACKer that is not fast enough (but one that is faster than the current ACKer), will result in the provider trying to find an even faster ACKer subsequently in the next period.
If the new ACKer is too fast, the provider can easily find a slower one based on the slower ACKer selection means described above. The provider can gradually find a proper sending rate using this mechanism.


\subsection{ACKer Logic}
\label{sec-pubcontrol-acker}
%\mnote{we could move this to come after ACKer Selection and probably as the first part of the ACKer shift section}
%Jia: The "ask for all" logic will be used by the ACKer selection... Was struggling about this also.
Since every packet sent from the data provider will be received by multiple receivers, the data provider places the ACKer ID in every data packet to assign a proper ACKer for that packet. On receiving a packet with his own ID, that receiver sends an ACK back to the data provider. Using a congestion control model like TCP, a closed feedback loop is thus formed between sender
and the ACKer to align the sending rate to the ACKer's receive rate.

Unlike the communication model of the followers, the rate is controlled on the sender (content provider) side for the ACKer (and thereby the
'faster' receivers forming the majority). The ACKer is likely to receive \emph{all} the packets for that flow. This is also achieved by modifying an Interest packet. We still put the flow ID in the Content Name field but
utilize a flag bit to indicate to intermediate router to forward all the packets in the flow to that outgoing face.


\subsection{ACKer Switching Policy}
\begin{figure}[t!]
  \centering
  \includegraphics[width=0.4\textwidth]{figures/ACKerShift}\\
  \caption{Procedure of ACKer shift}\label{fig:ackershift}
\end{figure}



%See if we have better reason why we use an in-band ACKer notification but not like the info collection
% Mayutan: we need to avoid using he, if we use it, it might be better to use (s)he of just she, her and etc..
To ensure the reliable method to switch between the new and the old ACKer, we designed an in-band notification procedure.
The procedure is shown in Fig.~\ref{fig:ackershift}. When the data provider decides to shift to a new ACKer at time $t1$, he starts to send packets indicating that both the original ACKer and the new ACKer should provide feedback (ACK). Since the new ACKer is still using the follower logic, he may miss some of these packets especially if he has a lower available bandwidth (the dashed lines on the right). But the new ACKer will eventually receive a data packet with his ID in the ACKer list. This is the first time the new ACKer sees his ID in the ACKer list. He will first change the request type to ``all'' by sending a special Interest packet described in \S\ref{sec-pubcontrol-acker}, and then send an ACK to the packet from the data provider.
Both the request to ``all'' and the ACK will follow the same path towards the data provider. So at time $t2$, when the data provider receives the ACK from the new ACKer (segment number might be larger than $S1$), the provider can be sure that the new ACKer is using the ACKer logic. From the next packet onwards (segment number $S2$), the provider sends data with only the new ACKer's ID.

We realize that for packets with segment number between $S1$ and $S2$, the new ACKer's ACKs are not reliable since during that period, the new ACKer can miss packets because it is using the follower logic. Receiving an
ACK from the new ACker for $S2$ ($t3$ in the figure) might also not indicate the end of the shift since the original ACKer might have a longer latency than the new one. To better control the provider window during this phase, we assign every packet an ACKer. For packets in range $[S1, S2)$, although both ACKers might receive and send an ACK, we only consider the original ACKer. The new ACKer's ACKs in that range will be discarded by the provider. For packets with segment number $\geq S2$, the provider will use the new ACKer.

}















% Removed the router-assisted part
\hide{

%Since the sending rate might also be application specific, \eg, audio/video streaming, we leave the rate choosing as an end-to-end behavior. This kind of design also helps reduce the states kept in the routers and increases the scalability of the solution. Here, we only provide one kind of the rate control mechanism that can satisfy general-purpose data transmissions. But the architecture is not limited to the solution. And for scalability (\ie, a flow having more than $10^6$ consumers), we also provide a router-assisted mechanism to help with information collection.



\subsection{Router-assisted ACKer Selection}

Sending all the periodical feedback towards the data provider might not be scalable enough. In a large scale dissemination where the number of receivers comes to $10^6$ or more, it is very difficult for the data provider to process such large amount of data and the solution might also incur heavy load in the network. To reduce the data collection workload, we provide a general router-assisted aggregation model. We call it general because the model is not limited to congestion control, it can be used in any communication that needs aggregation to reduce workload, \eg, sensor network, \etc.

\subsubsection{Histogram-based aggregation}

Like basic ACKer selection, the histogram-based aggregation also requires the data collector to trigger a collection phase. He needs to define: 1) requirement of the responder, 2) how many cells are there in the histogram, 3) how to calculate which cell a responder belongs to, and 4) what's the timeout for collection period.

This message will be published using COPSS and when it is disseminated to the routers, the routers create an entry to aggregate data.
When a responder (a receiver in the flow) receives the message, if he meets the requirement specified by the message, he calculates the cell he is in and responds with the cell ID.
After collecting the responses from all the outgoing links or when the timeout reaches, a router sends the aggregated data upstream. Note that the routers here don't have to understand the meaning of the histogram, just forward the list of cell ID and count upstream.

The calculation of timeout might be a difficult part in the aggregation method. The optimal case would be the routers can estimate the time span on every hop and reduce that value when disseminating to the next hop. But the value is difficult to measure due to the effect of queuing. For simplicity, we assume that every router reduces a constant value before it sends the aggregation request downstream, say $2ms$. But it can be optimized by RTT measurement mechanisms like \jnote{try to cite some}.

\subsubsection{Use of aggregation in congestion control}

Now, the data provider sends an aggregation collection message to all the receivers instead of the original control message. Normally when a periodical feedback request starts, the responder range is all the receivers. He also needs to specify the cells. Here, the cells are calculated by the receive rate, duplicate rate, and mark rate. Since the maximum receive rate is limited by the sending rate, the provider can specify cells according to that value.

After the timeout period, the data provider can receive a histogram that indicates the distribution of receive rate among all the data receivers. If the distribution is clear enough to identify the cell the ACKer is in, the data provider indicates that all the receivers in that cell should respond with their own ID. Then, the data provider selects the first responder as the ACKer.

If the distribution is not clear enough, \ie there are too many receivers in the cell the ACKer should be in, the data provider should initiate another histogram collection phase, in which only the receivers in that cell should respond. And he provides a fine-grained histogram. He keeps doing this until when the distribution is good enough to pick an ACKer. \jnote{Do we need to prove the upper bound of the selection phase?}
}

